BrackishMOT: The Brackish Multi-Object Tracking Dataset

There exist no publicly available annotated underwater multi-object tracking (MOT) datasets captured in turbid environments. To remedy this we propose the BrackishMOT dataset with focus on tracking schools of small fish, which is a notoriously difficult MOT task. BrackishMOT consists of 98 sequences captured in the wild. Alongside the novel dataset, we present baseline results by training a state-of-the-art tracker. Additionally, we propose a framework for creating synthetic sequences in order to expand the dataset. The framework consists of animated fish models and realistic underwater environments. We analyse the effects of including synthetic data during training and show that a combination of real and synthetic underwater training data can enhance tracking performance. Links to code and data can be found at https://www.vap.aau.dk/brackishmot

==> figures/synthDataEnv/compositeImg.tex <==
\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/synthDataEnv/null.png}
         \caption{Synth-brack}
         \label{fig:synthEnvBasis}
     \end{subfigure}
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/synthDataEnv/b.png}
         \caption{Synth-B-brack}
     \end{subfigure}
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/synthDataEnv/f.png}
         \caption{Synth-F-brack}
     \end{subfigure}
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/synthDataEnv/d.png}
         \caption{Synth-D-brack}
     \end{subfigure}
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/synthDataEnv/fd.png}
         \caption{Synth-FD-brack}
     \end{subfigure}
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/synthDataEnv/fb.png}
         \caption{Synth-BF-brack}
     \end{subfigure}
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/synthDataEnv/db.png}
         \caption{Synth-BD-brack}
     \end{subfigure}
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/synthDataEnv/fdb.png}
         \caption{Synth-BFD-brack}
     \end{subfigure}
        \caption{Visualisation of different conditions of our synthetic environment. \textbf{(a)} Plain background, no fog, no distractors. \textbf{(b)} Video background, no fog, no distractors. \textbf{(c)} Plain background, fog, no distractors. \textbf{(d)} Plain background, no fog, with distractors. \textbf{(e)} Plain background, with fog and distractors. \textbf{(f)} Video background with fog, but without distractors. \textbf{g} Video background with distractor, but without fog. \textbf{(g} Video background with fog and distractors. Best viewed in color and zoomed in.}
        \label{fig:synthEnv}
\end{figure*}

==> sections/ablation.tex <==
\subsection{Ablation Study of the Synthetic Environment}\label{sec:ablation}
In the development of synthetic data, it is possible to add and tweak features to make the data more or less realistic, complex, or noisy.
However, the benefits of such features are not always clear.
Therefore, we investigate how the combinations of turbidity (T), background (B), and distractors (D) affect the performance of the MS COCO and ImageNet pre-trained CenterTrack models.
There is a total of eight combinations, where, as an example, COCO-Synth$_{TD}$ is the MS COCO pre-trained CenterTrack model, which has then been fine-tuned on the synthetic sequences that have a plain background but includes turbidity and distractors.

The performances are presented in \tableref{synth_datasets} where the models have been evaluated on the BrackishMOT test split sequences that include the \textit{small fish} class (the sequences presented in \tableref{qualitative}).

%it is not always clear whether additional features affect the output in a positive manner.
%In this study, we investigate how the design of synthetic training data affects the performance of CenterTrack.
%Specifically, we take basis in a plain greenish environment with a single species of synthetic fish, that resembles the small fish of the Brackish Dataset.
%Our base environment is presented in \figref{synthEnvBasis}.
%As mentioned before, we add additional features to create variation in the dataset.
%This includes turbidity/fog, a complex background, and distractors.
%The three features, and all their combinations, are presented in \figref{synthEnv}.

%\include{figures/synthDataEnv/compositeImg}

%The background, synthetic fish, and combination of the two are presented in \figref{synthetic}.

%\begin{figure}[h]
%    \centering
%    \begin{subfigure}[b]{0.32\linewidth}
%    \includegraphics[width=\linewidth]{figures/placeholders/green.png}
%    \caption{Background}
%    \label{fig:green_background}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.32\linewidth}
%    \includegraphics[width=\linewidth]{figures/placeholders/fish.png}
%    \caption{Fish}
%    \label{fig:fish}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.32\linewidth}
%    \includegraphics[width=\linewidth]{figures/placeholders/green_fish.png}
%    \caption{Combined}
%    \label{fig:green_fish}
%    \end{subfigure}
%    \caption{Synthetic environment.}
%    \label{fig:synthetic}
%\end{figure}

%We add additional features to create variation in the dataset. This includes turbidity/fog, a complex background, and distractors. The three features are presented in \figref{synth_features}.
%This gives the possibility of creating six different types of environments depending on the number and types of features.
%In this ablation study we create eight synthetic datasets in eight different environments as presented in \tableref{synth_datasets}.
%In this ablation study we create eight synthetic datasets that are identical with respect to the number of fish and their swimming patterns, however, we change the environment around the fish as presented in \tableref{synth_datasets}.

%\begin{figure}[h]
%    \centering
%    \begin{subfigure}[b]{0.32\linewidth}
%    \includegraphics[width=\linewidth]{figures/placeholders/fog.png}
%    \caption{Fog}
%    \label{fig:fog}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.32\linewidth}
%    \includegraphics[width=\linewidth]{figures/placeholders/complex.png}
%    \caption{Complex}
%    \label{fig:complex}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.32\linewidth}
%    \includegraphics[width=\linewidth]{figures/placeholders/distractors.png}
%    \caption{Distractors}
%    \label{fig:distractors}
%    \end{subfigure}
%    \caption{Features to add on top of the synthetic environment to create different levels of variation.}
%    \label{fig:synth_features}
%\end{figure}

%\begin{table}[]
%\centering
%\caption{Performance of CenterTrack models trained on variations of the synthetic dataset. The performance of the models are measured on the small fish subset of the brackishMOT test split.}
%\label{tab:synth_datasets}
%\begin{tabular}{@{}lcccc@{}}
%\toprule
%Model & HOTA$\uparrow$ & MOTA$\uparrow$& IDF1$\uparrow$ \\ \midrule
%COCO-Synth        & 0.08 & -0.17 & 0.07  \\
%COCO-Synth$_B$      & 0.12 & -0.21 & 0.12  \\
%COCO-Synth$_T$      & 0.08 & -2.02 & 0.06  \\
%COCO-Synth$_D$     & 0.09 & -0.12 & 0.09  \\
%COCO-Synth$_{TD}$    & 0.12 & -0.14 & 0.12  \\
%COCO-Synth$_{BT}$   & 0.19 & 0.16 & 0.21  \\
%COCO-Synth$_{BD}$  & 0.15 & 0.08 & 0.16  \\
%COCO-Synth$_{BTD}$ & \textbf{0.21} & \textbf{0.18} & \textbf{0.24}  \\ \midrule
%ImNet-Synth       & 0.08 & -0.90 & 0.06  \\
%ImNet-Synth$_{B}$     & 0.14 & 0.05 & 0.17  \\
%ImNet-Synth$_{T}$     & 0.06 & -0.93 & 0.04  \\
%ImNet-Synth$_{D}$     & 0.08 & 0.03 & 0.08  \\
%ImNet-Synth$_{TD}$    & 0.06 & 0.02 & 0.05  \\
%ImNet-Synth$_{BT}$    & \textbf{0.19} & -0.24 & \textbf{0.21}  \\
%ImNet-Synth$_{BD}$    & 0.17 & \textbf{0.13} & 0.19  \\
%ImNet-Synth$_{BTD}$   & 0.13 & 0.00 & 0.14  \\ \bottomrule
%\end{tabular}
%\end{table}


\begin{table}[]
\centering
\caption{Performance of CenterTrack models trained on variations of the synthetic dataset. The performance of the models is measured on the small fish subset of the brackishMOT test split.}
\label{tab:synth_datasets}
\begin{tabular}{@{}lccc c lccc@{}}
\toprule
Model & HOTA$\uparrow$ & MOTA$\uparrow$& IDF1$\uparrow$ & & Model & HOTA$\uparrow$ & MOTA$\uparrow$& IDF1$\uparrow$ \\ \midrule
COCO-Synth        & 0.08 & -0.17 & 0.07 &\qquad\qquad &  ImNet-Synth & 0.08 & -0.90 & 0.06  \\
COCO-Synth$_B$  & 0.12 & -0.21 & 0.12 && ImNet-Synth$_{B}$     & 0.14 & 0.05 & 0.17  \\
COCO-Synth$_T$      & 0.08 & -2.02 & 0.06 &&  ImNet-Synth$_{T}$     & 0.06 & -0.93 & 0.04                         \\
COCO-Synth$_D$     & 0.09 & -0.12 & 0.09  &&  ImNet-Synth$_{D}$     & 0.08 & 0.03 & 0.08                          \\
COCO-Synth$_{TD}$    & 0.12 & -0.14 & 0.12&&  ImNet-Synth$_{TD}$    & 0.06 & 0.02 & 0.05                          \\
COCO-Synth$_{BT}$   & 0.19 & 0.16 & 0.21  &&  ImNet-Synth$_{BT}$    & \textbf{0.19} & -0.24 & \textbf{0.21}      \\
COCO-Synth$_{BD}$  & 0.15 & 0.08 & 0.16   &&  ImNet-Synth$_{BD}$    & 0.17 & \textbf{0.13} & 0.19                 \\
COCO-Synth$_{BTD}$ & \textbf{0.21} & \textbf{0.18} & \textbf{0.24}   &&  ImNet-Synth$_{BTD}$   & 0.13 & 0.00 & 0.14                           \\ \midrule
\end{tabular}
\end{table}

%\begin{table}[h]
%\centering
%\caption{ImageNet pre-trained CenterTrack models trained 10 epochs on synth followed by 30 epochs of training on the brackishMOT train split. Evaluated on the test subset containing small fish sequences.}
%\label{tab:synth_brack_datasets}
%\begin{tabular}{@{}lccc@{}}
%\toprule
%Model                 & HOTA$\uparrow$ & MOTA$\uparrow$& IDF1$\uparrow$ \\ \midrule
%CT-ImNet-Synth-brack     & 0.39 & 0.46 & 0.45 \\
%CT-ImNet-Synth-B-brack   & 0.38 & 0.45 & 0.43 \\
%CT-ImNet-Synth-T-brack   & 0.41 & \textbf{0.52} & \textbf{0.49} \\
%CT-ImNet-Synth-D-brack   & 0.41 & 0.49 & 0.47 \\
%CT-ImNet-Synth-TD-brack  & \textbf{0.42} & 0.47 & \textbf{0.49} \\
%CT-ImNet-Synth-BT-brack  & 0.41 & \textbf{0.52} & 0.48 \\
%CT-ImNet-Synth-BD-brack  & 0.41 & 0.51 & 0.48 \\
%CT-ImNet-Synth-BTD-brack & 0.41 & 0.51 & \textbf{0.49} \\ \bottomrule
%\end{tabular}
%\end{table}
%
%\begin{table}[h]
%\centering
%\caption{MS COCO pre-trained CenterTrack models trained 10 epochs on synth followed by 30 epochs of training on the brackishMOT train split. Evaluated on the test subset containing small fish sequences.}
%\label{tab:synth_brack_datasets}
%\begin{tabular}{@{}lccc@{}}
%\toprule
%Model                & HOTA$\uparrow$ & MOTA$\uparrow$& IDF1$\uparrow$ \\ \midrule
%CT-COCO-Synth-brack     & 0.39 & 0.46 & 0.44 \\
%CT-COCO-Synth-B-brack   & 0.38 & 0.47 & 0.44 \\
%CT-COCO-Synth-T-brack   & 0.38 & 0.43 & 0.44 \\
%CT-COCO-Synth-D-brack   & 0.39 & 0.50 & 0.44 \\
%CT-COCO-Synth-TD-brack  & 0.38 & 0.48 & 0.44 \\
%CT-COCO-Synth-BT-brack  & 0.36 & 0.42 & 0.41 \\
%CT-COCO-Synth-BD-brack  & 0.37 & 0.46 & 0.43 \\
%CT-COCO-Synth-BTD-brack & 0.39 & 0.47 & 0.44 \\ \bottomrule
%\end{tabular}
%\end{table}

==> sections/baseline.tex <==
It is notoriously difficult for humans to visually track fish of the same species in video sequences captured in the wild due to the similar appearance of the objects.
This is especially true when the water is turbid, the camera resolution is low, and the objects swim close to each other as is the case in some of the BrackishMOT sequences.
This indicates that visual cues for re-identifying the objects are not pronounced and likely not very reliable for solving this specific problem.
Therefore, we conduct experiments based on the state-of-the-art tracker CenterTrack~\cite{zhou2020tracking}, which tracks objects as points and focuses on associating objects locally between consecutive frames with little emphasis on visual features.

We present results based on different training strategies with and without the use of synthetic data, to investigate the potential benefit of using synthetic data in noisy underwater environments.
We evaluate our models based on conventional MOT performance metrics like the Multiple Object Tracking Accuracy metric (MOTA) from the CLEAR MOT metrics~\cite{bernardin2008evaluating}, the ID F1 score (IDF1)~\cite{ristani2016performance}, and the recent Higher Order Tracking Accuracy metric (HOTA)~\cite{luiten2021hota}.   

\subsection{Training}
As a basis for the experiments, we use two pre-trained models provided by the authors of CenterTrack and fine-tune on top of them to reduce training time and minimize the potential of overfitting. 
We name the CenterTrack models CT-COCO and CT-ImNet, where
CT-COCO has been pre-trained on the MS COCO~\cite{lin2014microsoft} dataset and CT-ImNet has been pre-trained on the ImageNet~\cite{deng2009imagenet} dataset.
Both models have a similar architecture with a DLA-34~\cite{yu2018deep} backbone.
The train and test splits of the BrackishMOT dataset consist of 78  and 20 sequences, respectively.

The models are fine-tuned following three training strategies: \textit{Brack}, \textit{Synth}, and \textit{Mix}. 
When following the \textit{Brack} strategy, we fine-tune the model on the BrackishMOT train split for 30 epochs.
The \textit{synth} strategy is comprised of pre-training on the synthetic data for 10 epochs followed by fine-tuning on the BrackishMOT train split for 30 epochs.
Lastly, the \textit{Mix} strategy is to fine-tune the model on a combination of the synthetic data and the BrackishMOT train split for 30 epochs.
All the models are trained with a batch size of 12 and a learning rate of 1.25e-4.
The images of the BrackishMOT and synthetic sequences have been resized and padded from 1920x1080 to 960x544 following the strategy proposed by the authors of CenterTrack~\cite{zhou2020tracking}.

\subsubsection{Choosing a Suitable Synthetic Environment}
We only train the \textit{Synth} and \textit{Mix} models using a single set of synthetic sequences to avoid potential overfitting.
To find the sequences best suited for increasing the performance of the trackers we conduct an ablation study, where we investigate how the combinations of the environment with turbidity (T), background (B), and distractors (D) affect the performance of the MS COCO and ImageNet pre-trained CenterTrack models.
The performances are presented in \tableref{synth_datasets} where the models have been evaluated on a sub-set of the BrackishMOT test split that only includes sequences of the \textit{small fish} class (the list of sequences is presented in \tableref{qualitative}).
We see that it is possible to train CenterTrack to be able to detect and track the \textit{small fish} class without ever seeing real images of the class.
The feature that seems to increase the tracking performance the most is the background videos whereas the turbidity and distractors give mixed results.

Based on the findings we pre-train the CT-COCO-Synth model on the Synth$_{BTD}$ sequences and the CT-ImNet-Synth on the Synth$_{BD}$ sequences followed by a fine-tuning on the BrackishMOT train split.
Both of the \textit{Mix} models are trained on a combined set of sequences consisting of the Synth$_{BTD}$ sequences and the BrackishMOT train split.



\begin{table}[]
\centering
\caption{Performance of CenterTrack models trained strictly on variations of the synthetic dataset. The performance of the models is measured on the subset of sequences from the BrackishMOT test split that contains the \textit{small fish} class.}
\label{tab:synth_datasets}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lccc c lccc@{}}
\toprule
\textbf{CT-COCO} & HOTA$\uparrow$ & MOTA$\uparrow$& IDF1$\uparrow$ & & \textbf{CT-ImNet} & HOTA$\uparrow$ & MOTA$\uparrow$& IDF1$\uparrow$ \\ \midrule
Synth        & 0.08 & -0.17 & 0.07 &\qquad\qquad &  Synth & 0.08 & -0.90 & 0.06  \\
Synth$_B$  & 0.12 & -0.21 & 0.12 && Synth$_{B}$     & 0.14 & 0.05 & 0.17  \\
Synth$_T$      & 0.08 & -2.02 & 0.06 &&  Synth$_{T}$     & 0.06 & -0.93 & 0.04                         \\
Synth$_D$     & 0.09 & -0.12 & 0.09  &&  Synth$_{D}$     & 0.08 & 0.03 & 0.08                          \\
Synth$_{TD}$    & 0.12 & -0.14 & 0.12&&  Synth$_{TD}$    & 0.06 & 0.02 & 0.05                          \\
Synth$_{BT}$   & 0.19 & 0.16 & 0.21  &&  Synth$_{BT}$    & \textbf{0.19} & -0.24 & \textbf{0.21}      \\
Synth$_{BD}$  & 0.15 & 0.08 & 0.16   &&  Synth$_{BD}$    & 0.17 & \textbf{0.13} & 0.19                 \\
Synth$_{BTD}$ & \textbf{0.21} & \textbf{0.18} & \textbf{0.24}   &&  Synth$_{BTD}$   & 0.13 & 0.00 & 0.14  \\ \midrule
\end{tabular*}
\end{table}

\subsection{Evaluation}
Quantitative performance results for the models are presented in \tableref{quantitative} for the test split and the 'small fish split'.
The small fish split is a subset of the test split that only contains the sequences with the \textit{small fish} class.
We use it to examine whether the models trained on the synthetic data overfit to the \textit{small fish} class.
Generally, we see a tendency that the ImageNet pre-trained models perform better than the models pre-trained on the MS COCO dataset, which indicates that the ImageNet dataset lays a stronger foundation for detecting the objects of the BrackishMOT dataset.
Furthermore, we see that the CT-COCO models do not really benefit from the synthetic data, which is surprising and in contrast to the results of the ablation study that showed how fine-tuning the CT-COCO model on the Synth$_{BTD}$ sequences resulted in the best performing synthetically trained tracker.

For the CT-ImNet-Synth$_{BT}$ model we see a slight decrease in MOTA and IDF1 when evaluating on the test split, but an increase in the \textit{small fish} sequences, this indicates that the model learns from the synthetic data to better track the \textit{small fish} objects but at the expense of some of the other classes.
When combining the real and synthetic data using the \textit{Mix} strategy, the CT-ImNet-Mix model exhibits similar performance as the CT-ImNet-Synth$_{BT}$ model on the \textit{small fish} sequences.
However, the performance is also generally increased when looking at all the test sequences, which indicates that the ability to track the other classes is maintained.
\begin{table}[]
\centering
\caption{Tracking results on the subset of the brackishMOT test sequences only containing the \textit{small fish} class.}
\label{tab:quantitative}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lclccc clccc@{}}
\toprule
Model                  &\qquad\qquad&& HOTA$\uparrow$ & MOTA$\uparrow$& IDF1$\uparrow$ &\quad\qquad&&  HOTA$\uparrow$ & MOTA$\uparrow$& IDF1$\uparrow$\\ \midrule
CT-COCO-Brack && \parbox[t]{5mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{Test split}}}} & 0.36 & 0.37 & 0.39 && \parbox[t]{5mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{Small fish split}}}}& 0.37 & 0.47 & 0.43 \\
CT-COCO-Synth$_{BTD}$  &&& 0.36 & 0.38 & 0.39 &&& 0.39 & 0.47 & 0.44 \\
CT-COCO-Mix            &&& 0.36 & 0.37 & 0.39 &&& 0.37 & 0.46 & 0.43 \\
CT-ImNet-Brack         &&& 0.38 & 0.43 & 0.44 &&& 0.39 & 0.50 & 0.46 \\
CT-ImNet-Synth$_{BT}$  &&& 0.38 & 0.42 & 0.41 &&& \textbf{0.41} & \textbf{0.52} & 0.48 \\
CT-ImNet-Mix           &&& \textbf{0.40} & \textbf{0.44} & \textbf{0.45} &&& \textbf{0.41} & \textbf{0.52} & \textbf{0.49} \\ \bottomrule
\end{tabular*}
\end{table}

In \tableref{qualitative} we present the results of the CT-ImNet-Mix model when evaluated on the small fish split.
In the table, we present additional metrics for the sequences to increase in order to better analyze the capabilities of the proposed model.
The additional metrics are detections (\textit{Dets}), ground truth detections (\textit{GT dets}), identities (\textit{IDs}), ground truth IDs (\textit{GT IDs}), and ID switches (\textit{IDSW}).

\begin{table}[]
\centering
\caption{Tracking results of the CT-ImNet-Mix model on the small fish split.}
\label{tab:qualitative}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lccccccccc@{}}
\toprule
Sequence        & HOTA$\uparrow$ & MOTA$\uparrow$& IDF1$\uparrow$ & Dets & GT dets & IDs & GT IDs & IDSW \\ \midrule
brackishMOT-50  & 0.40 & 0.46 & 0.47 & 1785 & 2129 & 105 &  17 & 50   \\
brackishMOT-55  & 0.35 & 0.46 & 0.43 & 2318 & 3192 & 187 &  37 & 112  \\
brackishMOT-56  & 0.53 & 0.41 & 0.75 & 80   & 87   & 7   &  1  & 4    \\
brackishMOT-67  & 0.18 & 0.11 & 0.10 & 173  & 636  & 31  &  4  & 7    \\
brackishMOT-90  & 0.61 & 0.53 & 0.74 & 401  & 426  & 18  &  3  & 7    \\
brackishMOT-93  & 0.44 & 0.51 & 0.51 & 1450 & 1567 & 160 &  45 & 82   \\ 
brackishMOT-95  & 0.44 & 0.38 & 0.39 & 619  & 148  & 28  &  1  & 0    \\ 
brackishMOT-98  & 0.49 & 0.58 & 0.60 & 1728 & 1930 & 137 &  36 & 80   \\ \bottomrule
\end{tabular*}
\end{table}

If we inspect the brackishMOT-93 and brackishMOT-95 sequences we see that they have 45 and 1 GT IDs, respectively. 
However, both sequences score a HOTA performance of 0.44 indicating that a higher number of objects does not seem to significantly impact the performance negatively.
This is emphasized by looking at BrackishMOT-67, which has only four GT IDs but the tracker only manages to get a HOTA score of 0.18.
If we inspect the BrackishMOT-67 sequence visually, we find that it has a single medium-sized object of the \textit{small fish} class, which the model tracks well throughout the sequence, however, there are also three very small objects of the \textit{small fish} class close to the seabed, which it has troubles finding and tracking.  

Another example where the tracker exhibits relatively low performance is on the brackishMOT-55 sequence.
However, if we inspect the sequence we see that the tracker only has difficulties detecting the fish against the patterned object in the background as illustrated in \figref{seq55}.
The patterned object is also part of sequences in the BrackishMOT train split and in some of the synthetic sequences that include the video background, however, it may be that the objects are less likely to appear in that region of the view, which would explain the weak detections.

\begin{figure}[]
    \centering
    \begin{subfigure}[t]{0.44\linewidth}
    \includegraphics[width=\textwidth]{figures/seq55-37.jpg} 
    \caption{BrackishMOT-55 frame 37.}
    \end{subfigure}
    \qquad
    \begin{subfigure}[t]{0.44\linewidth}
    \includegraphics[width=\textwidth]{figures/seq55-100.jpg} 
    \caption{BrackishMOT-55 frame 100.}
    \end{subfigure}
    \caption{Illustrative example of the performance of the CT-ImNet-Mix model, which is able to detect and track the fish well when they are not in front of the patterned obstacle.}
    \label{fig:seq55}
\end{figure}

==> sections/baseline_daniel.tex <==
It is notoriously difficult for humans to visually track fish of the same species in video sequences captured in the wild due to similar appearance of the objects. This is especially true when the water is turbid, the camera resolution is low, and the objects swim close to each other as it is the case in some of the BrackishMOT sequences. This indicates that visual cues for re-identifying the objects are not pronounced and likely not very reliable for solving this specific problem.
Therefore, we conduct experiments based on the state of the art tracker CenterTrack~\cite{zhou2020tracking}, which tracks objects as points and focuses on associating objects locally between consecutive frames with little emphasis on visual features. 

%As a basis for the experiments we use two pre-trained models provided by the authors of CenterTrack and fine-tune on top of them to reduce training time and minimize the potential of overfitting. We name the CenterTrack models CT-COCO and CT-ImNet, where CT-COCO has been pre-trained on the MS COCO~\cite{lin2014microsoft} dataset and CT-ImNet has been pre-trained on the ImageNet~\cite{deng2009imagenet} dataset. Both models have a similar architecture with a DLA-34~\cite{yu2018deep} backbone.

%We present results based on different training strategies with and without the use of synthetic data, to investigate the potential benefit of using synthetic data in noisy underwater environments.

We evaluate our models based on conventional MOT performance metrics like the Multiple Object Tracking Accuracy metric (MOTA) from the CLEAR MOT metrics~\cite{bernardin2008evaluating}, the ID F1 score (IDF1)~\cite{ristani2016performance}, and the recent Higher Order Tracking Accuracy metric (HOTA)~\cite{luiten2021hota}.

As a basis for the experiments, we use two pre-trained models provided by the authors of CenterTrack and fine-tune on top of them to reduce training time and minimize the potential of overfitting. We name the CenterTrack models CT-COCO and CT-ImNet, where CT-COCO has been pre-trained on the MS COCO~\cite{lin2014microsoft} dataset and CT-ImNet has been pre-trained on the ImageNet~\cite{deng2009imagenet} dataset. Both models have a similar architecture with a DLA-34~\cite{yu2018deep} backbone.
%The train and test splits of the BrackishMOT dataset consist of 78  and 20 sequences, respectively.

The models are fine-tuned following three training strategies: \textit{Brack}, \textit{Synth}, and \textit{Mix}. When following the \textit{Brack} strategy, we fine-tune the model on the BrackishMOT train split for 30 epochs. The \textit{Synth} strategy is comprised of pre-training on the synthetic data for 10 epochs followed by fine-tuning on the BrackishMOT train split for 30 epochs. Lastly, the \textit{Mix} strategy is to fine-tune the model on a combination of the synthetic data and the BrackishMOT train split for 30 epochs. \dale{We only train the \textit{Synth} and \textit{Mix} models using a single set of synthetic sequences to avoid potential overfitting.}

All the models are trained with a batch size of 12 and a learning rate of 1.25e-4. The images of the BrackishMOT and synthetic sequences have been resized and padded from 1920x1080 to 960x544 following the strategy proposed by the authors of CenterTrack~\cite{zhou2020tracking}.

%\dale{First, we present results achieved with the \textit{Brack} training strategy. Afterwards, we conduct ablation study, where we investigate how different environmental conditions affect the performance of the the pre-trained CenterTrack models. This is done in order to find the best performing set of synthetic sequences which will be then used with \textit{Synth} and \textit{Mix} strategies. We only train the \textit{Synth} and \textit{Mix} models using a single set of synthetic sequences to avoid potential overfitting. Finally, we present comparative results across all three strategies.}
%the potential benefit of using synthetic data in noisy underwater environments using using data generate in our synthetic environment, which consists of \textit{Synth} and \textit{Mix} strategies.

\subsection{Evaluation on the real world data only - \textit{Brack strategy}}
%Quantitative performance results for the models are presented in \tableref{realdata_quantitative} for the test split. Generally, we see a tendency that the ImageNet pre-trained models perform better than the models pre-trained on the MS COCO dataset, which indicates that the ImageNet dataset lays a stronger foundation for detecting the objects of the BrackishMOT dataset.

%Quantitative performance results for the models trained on only the real world data are presented in \tableref{quantitative} for the test split and the 'small fish split'. The small fish split is a subset of the test split that only contains the sequences with the \textit{small fish} class. We use this split to examine whether the models trained on the synthetic data overfits to the \textit{small fish} class. \dale{The list of sequences contained in the 'small fish split' is presented in \tableref{qualitative}.}

Quantitative performance results for both models trained solely on the proposed BrackishMOT dataset are presented in \tableref{realdata_quantitative}. The train and test splits of the BrackishMOT dataset consist of 78  and 20 sequences, respectively. \dale{Based on the results, we see that CT-ImNet outperforms CT-COCO model.}

\begin{table}[]
    \centering
    \caption{Tracking results achieved after training solely on the real world data.}
    \label{tab:realdata_quantitative}
    \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lccc@{}}
        \toprule
        Model                  & HOTA$\uparrow$ & MOTA$\uparrow$& IDF1$\uparrow$\\ \midrule
        CT-COCO-Brack  & 0.36 & 0.37 & 0.39  \\
        CT-ImNet-Brack & \textbf{0.38} & \textbf{0.43} & \textbf{0.44} \\
        \bottomrule
    \end{tabular*}
\end{table}

%\dale{Based on the results, we see that the ImageNet pre-trained model CT-ImNet performs better on the real world data than the CT-COCO model, which was pre-trained on the MS COCO dataset.}

\iffalse{
\begin{table}[]
    \centering
    \caption{Tracking results achieved after training solely on the real world data.}
    \label{tab:realdata_quantitative}
    \begin{tabular}{lllllcccllllccc}
        \multicolumn{1}{c}{} &  &  &  &  & \multicolumn{3}{c}{\textbf{Test Split}} &  &  &  &  & \multicolumn{3}{c}{\textbf{Small fish split}} \\ \hline
        Model &  &  &  &  & \multicolumn{1}{l}{HOTA$\uparrow$} & \multicolumn{1}{l}{MOTA$\uparrow$} & \multicolumn{1}{l}{IDF1$\uparrow$} &  &  &  &  & \multicolumn{1}{l}{HOTA$\uparrow$} & \multicolumn{1}{l}{MOTA$\uparrow$} & \multicolumn{1}{l}{IDF1$\uparrow$} \\ \hline
        CT-COCO-Brack &  &  &  &  & 0.36 & 0.37 & 0.39 &  &  &  &  & 0.37 & 0.47 & 0.43 \\ \hline
        CT-ImNet-Brack &  &  &  &  & \textbf{0.38} & \textbf{0.43} & \textbf{0.44} &  &  &  &  & \textbf{0.39} & \textbf{0.50} & \textbf{0.46} \\ \hline
    \end{tabular}
\end{table}
}\fi






\subsection{Ablation study}
To find the sequences best suited \dale{for \textit{Synth} and \textit{Mix} strategies}, we conduct an ablation study, where we investigate how the combinations of the environment with turbidity (T), background (B), and distractors (D) affect the performance of the MS COCO and ImageNet pre-trained CenterTrack models.
The performances are presented in \tableref{synth_datasets} where the models have been evaluated on the sub-set of the BrackishMOT test split called 'small fish split'  which only contains the sequences with the \textit{small fish} class. The list of sequences contained in the 'small fish split' is presented in \tableref{qualitative}. 

We see that it is possible to train CenterTrack to be able to detect and track the \textit{small fish} class without ever seeing real images of the class.
The feature that seems to increase the tracking performance the most is the background videos whereas the turbidity and distractors give mixed results.

\dale{Based on the findings, we pre-train the CT-COCO-Synth model on the Synth$_{BTD}$ sequences and the CT-ImNet-Synth on the Synth$_{BD}$ sequences followed by a fine-tuning on the BrackishMOT train split. However, \textit{Mix} models are trained on a combined set of the Synth$_{BTD}$ sequences and the BrackishMOT train split. }

%Based on the findings we pre-train the CT-COCO-Synth model on the Synth$_{BTD}$ sequences and the CT-ImNet-Synth on the Synth$_{BD}$ sequences followed by a fine-tuning on the BrackishMOT train split.Both of the \textit{Mix} models are trained on a combined set of sequences consisting of the Synth$_{BTD}$ sequences and the BrackishMOT train split.

\begin{table}[]
\centering
\caption{Performance of CenterTrack models trained strictly on variations of the synthetic dataset. The performance of the models are measured on the 'small fish split'.}
\label{tab:synth_datasets}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lccc c lccc@{}}
\toprule
\textbf{CT-COCO} & HOTA$\uparrow$ & MOTA$\uparrow$& IDF1$\uparrow$ & & \textbf{CT-ImNet} & HOTA$\uparrow$ & MOTA$\uparrow$& IDF1$\uparrow$ \\ \midrule
Synth        & 0.08 & -0.17 & 0.07 &\qquad\qquad &  Synth & 0.08 & -0.90 & 0.06  \\
Synth$_B$  & 0.12 & -0.21 & 0.12 && Synth$_{B}$     & 0.14 & 0.05 & 0.17  \\
Synth$_T$      & 0.08 & -2.02 & 0.06 &&  Synth$_{T}$     & 0.06 & -0.93 & 0.04                         \\
Synth$_D$     & 0.09 & -0.12 & 0.09  &&  Synth$_{D}$     & 0.08 & 0.03 & 0.08                          \\
Synth$_{TD}$    & 0.12 & -0.14 & 0.12&&  Synth$_{TD}$    & 0.06 & 0.02 & 0.05                          \\
Synth$_{BT}$   & 0.19 & 0.16 & 0.21  &&  Synth$_{BT}$    & \textbf{0.19} & -0.24 & \textbf{0.21}      \\
Synth$_{BD}$  & 0.15 & 0.08 & 0.16   &&  Synth$_{BD}$    & 0.17 & \textbf{0.13} & 0.19                 \\
Synth$_{BTD}$ & \textbf{0.21} & \textbf{0.18} & \textbf{0.24}   &&  Synth$_{BTD}$   & 0.13 & 0.00 & 0.14  \\ \midrule
\end{tabular*}
\end{table}

\subsection{Comparative evaluation across all three training strategies}
Quantitative performance results for the models trained across all three strategies are presented in \tableref{quantitative} for both the test split and the 'small fish split'. We use the 'small fish split' to examine whether the models trained on the synthetic data overfits the \textit{small fish} class. 
%As previously mentioned, he small fish split is a subset of the test split that only contains the sequences with the \textit{small fish} class. We use it to examine whether the models trained on the synthetic data overfits to the \textit{small fish} class. 

Generally, we see a tendency that the ImageNet pre-trained models perform better than the models pre-trained on the MS COCO dataset, which indicates that the ImageNet dataset lays a stronger foundation for detecting the objects of the BrackishMOT dataset. Furthermore, we see that the CT-COCO models do not really benefit from the synthetic data, which is surprising and in contrast to the results of the ablation study that showed how fine-tuning the CT-COCO model on the Synth$_{BTD}$ sequences resulted in the best performing synthetically trained tracker.

For the CT-ImNet-Synth$_{BT}$ model we see a slight decrease in MOTA and IDF1 when evaluating on the test split, but an increase in the \textit{small fish} sequences. This indicates that the model learns from the synthetic data to better track the \textit{small fish} objects but at the expense of some of the other classes.
When combining the real and synthetic data using the \textit{Mix} strategy, the CT-ImNet-Mix model exhibits similar performance as the CT-ImNet-Synth$_{BT}$ model on the \textit{small fish} sequences.
However, the performance is also generally increased when looking at all the test sequences, which indicates that the ability to track the other classes is maintained.
\begin{table}[]
    \centering
    \caption{Tracking results on the subset of the brackishMOT test sequences only containing the \textit{small fish} class.}
    \label{tab:quantitative}
    \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lclccc clccc@{}}
        \toprule
        Model                  &\qquad\qquad&& HOTA$\uparrow$ & MOTA$\uparrow$& IDF1$\uparrow$ &\quad\qquad&&  HOTA$\uparrow$ & MOTA$\uparrow$& IDF1$\uparrow$\\ \midrule
        CT-COCO-Brack && \parbox[t]{5mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{Test split}}}} & 0.36 & 0.37 & 0.39 && \parbox[t]{5mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{Small fish split}}}}& 0.37 & 0.47 & 0.43 \\
        CT-COCO-Synth$_{BTD}$  &&& 0.36 & 0.38 & 0.39 &&& 0.39 & 0.47 & 0.44 \\
        CT-COCO-Mix            &&& 0.36 & 0.37 & 0.39 &&& 0.37 & 0.46 & 0.43 \\
        CT-ImNet-Brack         &&& 0.38 & 0.43 & 0.44 &&& 0.39 & 0.50 & 0.46 \\
        CT-ImNet-Synth$_{BT}$  &&& 0.38 & 0.42 & 0.41 &&& \textbf{0.41} & \textbf{0.52} & 0.48 \\
        CT-ImNet-Mix           &&& \textbf{0.40} & \textbf{0.44} & \textbf{0.45} &&& \textbf{0.41} & \textbf{0.52} & \textbf{0.49} \\ \bottomrule
    \end{tabular*}
\end{table}

In \tableref{qualitative} we present the results of the CT-ImNet-Mix, \dale{the best-performing model for both splits} when evaluated on the small fish split.
In the table, we present additional metrics for the sequences to better analyze the capabilities of the proposed model.
The additional metrics are detections (\textit{Dets}), ground truth detections (\textit{GT dets}), IDs, ground truth IDs (\textit{GT IDs}), and ID switches (\textit{IDSW}).

\begin{table}[]
\centering
\caption{Tracking results of the CT-ImNet-Mix model on the small fish split.}
\label{tab:qualitative}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lccccccccc@{}}
\toprule
Sequence        & HOTA$\uparrow$ & MOTA$\uparrow$& IDF1$\uparrow$ & Dets & GT dets & IDs & GT IDs & IDSW \\ \midrule
brackishMOT-50  & 0.40 & 0.46 & 0.47 & 1785 & 2129 & 105 &  17 & 50   \\
brackishMOT-55  & 0.35 & 0.46 & 0.43 & 2318 & 3192 & 187 &  37 & 112  \\
brackishMOT-56  & 0.53 & 0.41 & 0.75 & 80   & 87   & 7   &  1  & 4    \\
brackishMOT-67  & 0.18 & 0.11 & 0.10 & 173  & 636  & 31  &  4  & 7    \\
brackishMOT-90  & 0.61 & 0.53 & 0.74 & 401  & 426  & 18  &  3  & 7    \\
brackishMOT-93  & 0.44 & 0.51 & 0.51 & 1450 & 1567 & 160 &  45 & 82   \\ 
brackishMOT-95  & 0.44 & 0.38 & 0.39 & 619  & 148  & 28  &  1  & 0    \\ 
brackishMOT-98  & 0.49 & 0.58 & 0.60 & 1728 & 1930 & 137 &  36 & 80   \\ \bottomrule
\end{tabular*}
\end{table}

If we inspect the brackishMOT-93 and brackishMOT-95 sequences we see that they have 45 and 1 GT IDs, respectively. 
However, both sequences score a HOTA performance of 0.44 indicating that a higher number of objects does not seem to significantly impact the performance negatively.
This is emphasized by looking at BrackishMOT-67, which have only four GT IDs but the tracker only manages to get a HOTA score of 0.18.
If we inspect the BrackishMOT-67 sequence visually, we find that it has a single medium-sized object of the \textit{small fish} class, which the model tracks well throughout the sequence, however, there are also three very small objects of the \textit{small fish} class close to the seabed, which it has troubles finding and tracking.  

Another example where the tracker exhibits relatively low performance is on the brackishMOT-55 sequence.
However, if we inspect the sequence we see that the tracker only has difficulties detecting the fish against the patterned object in the background as illustrated in \figref{seq55}.
The patterned object is also part of sequences in the BrackishMOT train split and in some of the synthetic sequences that include the video background, however, it may be that the objects are less likely to appear in that region of the view, which would explain the weak detections.

\begin{figure}[]
    \centering
    \begin{subfigure}[t]{0.44\linewidth}
    \includegraphics[width=\textwidth]{figures/seq55-37.jpg} 
    \caption{BrackishMOT-55 frame 37.}
    \end{subfigure}
    \qquad
    \begin{subfigure}[t]{0.44\linewidth}
    \includegraphics[width=\textwidth]{figures/seq55-100.jpg} 
    \caption{BrackishMOT-55 frame 100.}
    \end{subfigure}
    \caption{Illustrative example of the performance of the CT-ImNet-Mix model, which is able to detect and track the fish well when they are not in front of the patterned obstacle.}
    \label{fig:seq55}
\end{figure}

==> sections/discussion.tex <==
discuss
